Skills and Liquidity Barriers to Youth Employment: Medium-term Evidence from a Cash Benchmarking Experiment in Rwanda

We present results of an experiment benchmarking a workforce training program against cash transfers for underemployed young adults in Rwanda. 3.5 years after treatment, the training program enhances productive time use and asset investment, while the cash transfers drive productive assets, livestock values, savings, and subjective well-being. Both interventions have powerful effects on entrepreneurship. But while labor, sales, and profits all go up, the implied wage rate in these businesses is low. Our results suggest that credit is a major barrier to self-employment, but deeper reforms may be required to enable entrepreneurship to provide a transformative pathway out of poverty.

==> costing.tex <==
\begin{tabular}{l c c c c c c}
\toprule %
Treatment             Arm:	&	Ex Ante Cost	&	Value received 	&	Ex Post Cost	&	Fraction  operating cost 	&	Compliance Rate 	&	Cost per study household	\\
Huguka Dukore	&	\$464.25	&	\$153.47	&	\$388.32	&	60.5\%	&	85.6\%	&	\$332.27	\\
GD lower	&	\$377.03	&	\$317.16	&	\$394.39	&	19.6\%	&	100\%	&	\$394.39	\\
GD mid	&	\$464.25	&	\$410.65	&	\$493.96	&	16.9\%	&	99.4\%	&	\$490.99	\\
GD upper	&	\$571.74	&	\$502.96	&	\$590.41	&	14.8\%	&	100\%	&	\$590.41	\\
GD large	&	\$828.47	&	\$750.3	&	\$846.71	&	11.3\%	&	100\%	&	\$846.71	\\
Combined	&	\$928.5	&	\$561.11	&	\$885.64	&	36.3\%	&	89.6\%(HD), 100\%(GD)	&	\$840.20	\\

\bottomrule %
\end{tabular}

